SPEEDEX: A Scalable, Parallelizable, and Economically Efficient Decentralized EXchange

SPEEDEX is a decentralized exchange (DEX) that lets participants securely trade assets without giving any single party undue control over the market. SPEEDEX offers several advantages over prior DEXes. It achieves high throughput -- over 200,000 transactions per second on 48-core servers, even with tens of millions of open offers. SPEEDEX runs entirely within a Layer-1 blockchain, and thus achieves its scalability without fragmenting market liquidity between multiple blockchains or rollups. It eliminates internal arbitrage opportunities, so that a direct trade from asset $\mathcal{A}$ to asset $\mathcal{B}$ always receives as good a price as trading through some third asset such as USD. Finally, it prevents certain front-running attacks that would otherwise increase the effective bid-ask spread for small traders. SPEEDEX's key design insight is its use of an Arrow-Debreu exchange market structure that fixes the valuation of assets for all trades in a given block of transactions. We construct an algorithm, which is both asymptotically efficient and empirically practical, that computes these valuations while exactly preserving a DEX's financial correctness constraints. Not only does this market structure provide fairness across trades, but it also makes trade operations commutative and hence efficiently parallelizable. SPEEDEX is prototyped but not yet merged within the Stellar blockchain, one of the largest Layer-1 blockchains.

==> arrowdebreu.tex <==
\section{Arrow-Debreu Exchange Markets}
\label{apx:arrow}





==> extensions.tex <==
\section{Extensions}
\label{sec:extensions}

Ramseyer et al. \cite{ramseyer2022batch} show how to integrate
so-called Constant Function Market Makers (CFMMs) \cite{angeris2019analysis}
into the Arrow-Debreu exchange market framework, meaning that they could
be integrated smoothly into \Tat{}.
%Many automated market makers, such as those based on Uniswap's
%constant product rule \cite{uniswapv2}, integrate naturally
%into \SPEEDEX{} and do not require substantive changes to \Tat{} \cite{cfmmpreprint}.
\TheSDF{}'s deployment will make this integration with its own CFMMs.

\SPEEDEX{} does not implement offers to buy a fixed amount of an asset
 (e.g. buy at most 100 USD, spending as few EUR as possible).
 Buy offers admit the same logarithmic transformation as in \S \ref{sec:logtransform},
but in fact, these offers make the price computation
 problem PPAD-hard, a complexity class that is widely conjectured to
 be algorithmically intractable in polynomial time (\S \ref{sec:ppad}).
One could compute prices using only sell offers, and integrate buy offers in the linear programming step.

%Empirically, \Tat{} might be able handle a small number of buy offers.  Buy offers admit the same logarithmic transformation as in 
%\S \ref{sec:logtransform}.
%Alternatively, one could compute prices only using sell offers, and then integrate buy offers in the linear programming step.

\iffalse

The primary theoretical requirement for \Tat{} is that the market satisfy a property known as ``Weak Gross Substitutability'' (WGS).
Simply put, raising the price of one good should not decrease the net purchased amount of a different good (see \cite{codenotti2005market}).
Many natural types of trade offers, such as offers to sell multiple types of goods and/or acquire any one of multiple digital assets 
(e.g., trading many digital assets that are all backed by the same real-world currency) satisfy this property.

Many automated market makers, such as those based on Uniswap's
constant product rule \cite{uniswapv2}, can be formulated as an agent
that offers to sell an infinitesimal amount of a good at each price
point.  These market makers can therefore integrate naturally with
SPARROW-DEX, without modification to the underlying mathematics or to
\Tat.  \TheSDF{} will integrate constant-product market makers with
SPARROW-DEX.

SPARROW-DEX does not implement offers to buy a fixed amount of an asset (e.g., buy up to 100 USD, spending as few EUR as possible).
These offers do not satisfy WGS, and move the price computation problem from a complexity class that admits polynomial-time algorithms to one that is widely conjectured to be intractable.

\fi


